Unilateral Ground Contact Force Regulations in Thruster-Assisted Legged Locomotion

In this paper, we study the regulation of the Ground Contact Forces (GRF) in thruster-assisted legged locomotion. We will employ Reference Governors (RGs) for enforcing GRF constraints in Harpy model which is a bipedal robot that is being developed at Northeastern University. Optimization-based methods and whole body control are widely used for enforcing the no-slip constraints in legged locomotion which can be very computationally expensive. In contrast, RGs can enforce these constraints by manipulating joint reference trajectories using Lyapunov stability arguments which can be computed much faster. The addition of the thrusters in our model allows to manipulate the gait parameters and the GRF without sacrificing the locomotion stability.

==> unused.tex <==



\begin{comment}

    Implemented ERG framework suing the appropriate Lyapunov function and constraints:
    
    \begin{equation}V=(\boldsymbol{x}-\boldsymbol{x} \omega)^{\top} P\left(\boldsymbol{x}-\boldsymbol{x}_{w}\right)\end{equation}
    
    \begin{equation}\boldsymbol{x}=\left[\begin{array}{c}
    \boldsymbol{c} \\
    \dot{c}
    \end{array}\right] \quad \boldsymbol{x}_{\omega}=\left[\begin{array}{c}
    \dot{c} d \\
    \boldsymbol{w}
    \end{array}\right] \quad p>0\end{equation}
    
    The ground reaction forces $\boldsymbol{\lambda}$ are described by:
    
    \begin{equation}
    m\ddot{c}=R_{2}(\gamma)\left[\begin{array}{c}
    f_{x}^{\prime \prime} \\
    f_{y}^{\prime \prime} \\
    f_{z}-m g
    \end{array}\right]+\boldsymbol{\lambda}\end{equation}
    
    \begin{equation}\boldsymbol{\lambda}=m\boldsymbol{\ddot{c}} -R z(\gamma)\left(-m \boldsymbol{g}+\boldsymbol{f}_{T}^{\prime \prime}\right)\end{equation}
    
    Ground reaction force constraints:
    
    \begin{equation}\begin{aligned}
    |\lambda x| & \leq \mu_{5} \lambda_{z} \\
    \left|\lambda_{y}\right| & \leq \mu_{5} \lambda_{z} \\
    \lambda_{z} &>0
    \end{aligned}\end{equation}


\subsection{Kinematics}

The frames of reference of the system are defined below, where $\{x\}$, $\{x\}^{B}$, $\{x\}^{HL}$, $\{x\}^{HR}$ are the inertial, body, left hip, and right hip frames respectively, where $R_{B}$ is the body rotation matrix and $\gamma_{HL}$ is the frontal hip angle: 

\begin{equation}
\begin{aligned}
&\{x\} \\
&\{x\}^{B} = R_{B}^{\top} \{{x}\} \\
&\{x\}^{HL} = R_{x} (\gamma_{HL})^{\top} \{{x}\}^{B} \\
&\{x\}^{HR} = R_{x} (\gamma_{HR})^{\top} \{{x}\}^{B}
\end{aligned}
\end{equation}

The leg length vectors are defined below, where $\boldsymbol{l}_{1}^B$, $\boldsymbol{l}_{2}^{HL}$ and, $\boldsymbol{l}_{3}^{HL}$ are the vector from the body frame to the hip, from the frontal hip joint to the sagittal hip joint, and from the sagittal hip joint to the knee joint respectively. $\phi_{h}$ represents the sagittal hip angle:

\begin{equation}
\begin{aligned}
\boldsymbol{l}_{1}^B =
\begin{bmatrix}
l_{11}^B\\l_{12}^B\\l_{13}^B
\end{bmatrix} & \; \; \boldsymbol{l}_{2}^H =
\begin{bmatrix}
0\\l_{2}^H\\0
\end{bmatrix} & \boldsymbol{l}_{3}^H =
R_{y}(\phi_{h})
\begin{bmatrix}
0\\0\\l_{3}
\end{bmatrix}
\end{aligned}
\end{equation}

The leg parallel mechanism is defined as the following, where $\phi_{k}$ represents the knee angle:

\begin{equation}
\boldsymbol{l}_{4}^H = R_{y}(\phi_{h}) \begin{bmatrix}
-l_{4a}\cos\phi_{k} \\ 0 \\ -(l_{4b} + l_{4a} \sin{\phi_{k}})
\end{bmatrix}
\end{equation}

The inertial positions of the system $\boldsymbol{x}_{B}$, $\boldsymbol{x}_{P}$, $\boldsymbol{x}_{H}$, $\boldsymbol{x}_{K}$, $\boldsymbol{x}_{F}$ are the body, pelvis, hip, knee, and foot positions respectively, are defined below:

\begin{equation}
\begin{aligned}
&\boldsymbol{x}_{B} \\
&\boldsymbol{x}_{P} = \boldsymbol{x}_{B} + R_{B} \boldsymbol{l}_{1}^{B} \\
&\boldsymbol{x}_{H} =  \boldsymbol{x}_{P} + R_{B} R{x}(\gamma_{h}) \boldsymbol{l}_{2}^{H}\\
&\boldsymbol{x}_{K} = \boldsymbol{x}_{H} + R_{B} R{x}(\gamma_{h}) \boldsymbol{l}_{3}^{H}\\
&\boldsymbol{x}_{F} = \boldsymbol{x}_{k} + R_{B} R{x}(\gamma_{h}) \boldsymbol{l}_{4}^{H}
\end{aligned}
\end{equation}

Local angular velocities of the actuators are defined as the following, where  $\boldsymbol{\Omega}_{B}$, $\boldsymbol{\Omega}_{H}$, and $\boldsymbol{\Omega}_{K}$ are the body, pelvis, and hip angular velocities respectively:

\begin{equation}
\begin{aligned}
&\boldsymbol{\Omega}_{B} = \boldsymbol{\omega}_{B}^{B} \\
&\boldsymbol{\Omega}_{H} = \boldsymbol{\omega}_{P}^{B} + R_{B}^{\top} \omega_{B}^{B} \\
&\boldsymbol{\Omega}_{K} =  \boldsymbol{\omega}_{H}^{H} + \omega_{P}^{H} + R_{B}^{\top} \omega_{B}^{B} \end{aligned}
\end{equation}




\subsection{Dynamic modeling}

The linear and angular kinetic energies of the system $K_{L}$ and $K_{A}$ are defined as: 

\begin{equation}
K_{L}=\frac{1}{2}(m_{B} \dot{\boldsymbol{x}}_{B}^{\top} \dot{\boldsymbol{x}}_{B} + m_{H} \dot{\boldsymbol{x}}_{H}^{\top} \dot{\boldsymbol{x}}_{H} + m_{K} \dot{\boldsymbol{x}}_{K}^{\top} \dot{\boldsymbol{x}}_{K})
\end{equation}

\begin{equation}
K_{A}=\frac{1}{2}(\boldsymbol{\Omega}_{B}^{\top} \hat{I}_{B} \boldsymbol{\Omega}_{B} + \boldsymbol{\Omega}_{H}^{\top} \hat{I}_{H} \boldsymbol{\Omega}_{H} + \boldsymbol{\Omega}_{K}^{\top} \hat{I}_{K} \boldsymbol{\Omega}_{K})
\end{equation}

The potential energy $U$ of the system is defined as:

\begin{equation}
U = -\begin{bmatrix}
0 & 0 & g
\end{bmatrix} (m_{B}\boldsymbol{x}_{B} + m_{H}\boldsymbol{x}_{H} + m_{K}\boldsymbol{x}_{K})
\end{equation}

The Lagrangian function $L$ is defined as:
\begin{equation}
L = K_{L} + K_{A} - U
\end{equation}

The body angular velocity $\boldsymbol{\tau}_B$ and rotation $R_B$ in SO(3) are defined as:

\begin{equation}
\boldsymbol{\tau}_B = \frac{d}{dt} \bigg( \frac{\partial L}{\partial \boldsymbol{\Omega}_B} \bigg) + \boldsymbol{\Omega}_B \times \frac{\partial L}{\partial \boldsymbol{\Omega}_B} + \sum_{i=1}^{3} \boldsymbol{r}_i \times \frac{\partial L}{\partial \boldsymbol{r}_i}
\end{equation}

\begin{equation}
\frac{d}{dt} R_B = R_B [\boldsymbol{\Omega}_B]_x
\end{equation}

Remaining states:

\begin{equation}
\boldsymbol{u}_d = \frac{d}{dt} \bigg( \frac{\partial L}{\partial \dot{\boldsymbol{q}}_d} \bigg) - \frac{\partial L}{\partial \boldsymbol{q}_d}
\end{equation}

Massed dynamics:
\begin{equation}
\boldsymbol{q}_d = \begin{bmatrix}
\boldsymbol{x}_B & \gamma_{HL} & \phi_{HL} & \gamma_{HR} & \phi_{HR}
\end{bmatrix} ^\top
\end{equation}

Massless system:

\begin{equation}
\boldsymbol{u}_k = \begin{bmatrix}
\ddot{\phi}_{KL} \\
\ddot{\phi}_{KR}
\end{bmatrix}
\end{equation}

Combining equations into the following form:

\begin{equation}
M \dot{\boldsymbol{q}}_2 + \boldsymbol{h} = \boldsymbol{u}
\end{equation}

$\boldsymbol{q}_1$ and $\boldsymbol{q}_2$ are defined as the following

\begin{equation}
\boldsymbol{q}_1 = \begin{bmatrix}
\boldsymbol{q}_d & \boldsymbol{q}_k & \boldsymbol{r}_1 & \boldsymbol{r}_2 & \boldsymbol{r}_3
\end{bmatrix} ^\top
\end{equation}

\begin{equation}
\boldsymbol{q}_2 = \begin{bmatrix}
{\Omega}_{B} \\
\dot{q}_{d}
\end{bmatrix}
\end{equation}

The following equation of motion is used in the simulation:

\begin{equation}
\dot{\boldsymbol{x}} = \boldsymbol{f} ( \boldsymbol{x}, \boldsymbol{\tau}, \boldsymbol{u}_d, \boldsymbol{u}_k )
\end{equation}

\subsection{Constraints acting on the system}

Kinematic constraint using Lagrangian multiplier:

\begin{equation}
J_{s} \dot{\boldsymbol{q}}_{2} = \boldsymbol{h}_{c}
\end{equation}

Solution:
\begin{equation}
\begin{bmatrix}
M & {-J_{s}}^\top \\
J_{s} & 0
\end{bmatrix}
\begin{bmatrix}
\dot{\boldsymbol{q}}_{2}\\
\boldsymbol{\lambda}
\end{bmatrix}
= \boldsymbol{h}_{c}
\end{equation}

The ground friction constraint $\ddot{\boldsymbol{x}}_{F}=0$, which assumes the foot remains completely stationary, produces the following equation:

\begin{equation}
\dot{\boldsymbol{q}}_{2} + \dot{J}_{s} \boldsymbol{q}_{2} = 0
\end{equation}













The same GRFground reaction force constraint is defined as follows
%
\begin{equation}
    \begin{gathered}
    \bm h_r = \bm S \, \bm u_g + [0,0,-20]^\top \geq 0 \\
    \bm S = \begin{bmatrix}
    -\mathrm{sign}(u_{g,x}) & 0 & \mu_s \\
    0 & -\mathrm{sign}(u_{g,y}) & \mu_s \\
    0 & 0 & 1
    \end{bmatrix}
    \end{gathered}
\label{eq:ground_constraint}
\end{equation}

\section{Gait Design}

\textcolor{blue}{Content:
\begin{itemize}
    \item Implementing center of pressure to design the gait, which follows the formulation in Apggar's paper. Or we use the planar gait design to be stabilized with thrusters.
    \item Brief overview and algorithm to generate this gait.
\end{itemize}
}


\section{Controller Design}

\textcolor{blue}{Content:
\begin{itemize}
    \item Controller for the joints.
    \item Controller for stabilizing the 3D dynamics of the robot using thrusters.
    \item ERG optimization framework.
\end{itemize}
}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{img/harpyMechanical.eps}
    \caption{Harpy robot mechanical overview. Thrusters are rotated about the sagittal axis and are used to manipulate the gait dynamics to improve the robustness of the bipedal walking gait.}
    \label{fig:harpyMechanical}
\end{figure}

\begin{equation}
    \begin{aligned}
    \bm u_{t,c} &= (\bm I - \bm Y)(\bm K_{pt}(\bm c_t - \bm c) + \bm K_{dt}(\dot{\bm c_t} - \dot{\bm c})) \\
    u_r &= \bm J_s^\top (k_{pr}(\bm c_t - \bm c) + k_{dr}(\dot{\bm c_t} - \dot{\bm c})) \\
    \bm Y &= \bm J_s(\bm J_s^\top \bm J_s)^{-1}\bm J_s^\top,
    \end{aligned}
\label{eq:thruster_feedback_law}
\end{equation}


\end{comment}



%===============================================================
\section{Mechanical Design}

Harpy (Fig.~\ref{fig:midget}) is designed with the goal of being as lightweight, robust, and energy-dense as possible, which drives the use of carbon fiber composites and powerful thrusters and actuators. The upper body frame is printed with Markforged composite FDM 3D printing, which embeds continuous carbon fiber within the thermoplastic composite structure, producing lightweight and extremely robust parts. This part joins the lower body, amplifier rack, and thrusters while housing any additional electronics such as an IMU, a real-time computer, batteries, any other sensors.

The amplifier rack is primarily made up of a carbon fiber tube support structure that attaches to the upper body frame and a carbon fiber plate in which the amplifiers and their copper heatsinks are embedded. The heatsinks are held in place by a combination of carbon fiber plates and 3D printed supports in order to avoid the use of metal fasteners, reducing overall weight.

The leg links use custom-profile carbon fiber tubes, which are rectangular in cross-section in order to have optimal bending and torsional stiffness when compared to circular tubes. Smaller circular cross-section tubes are used for the 4-bar linkage control rod and feet due to their lesser need for torsional stiffness in order to reduce weight. The carbon fiber tubes are secured to the actuators and joints with a combination of flathead and set screws.

The hip-frontal, hip-sagittal, knee, and thruster actuators are virtually identical outside of slight geometry differences to accommodate different carbon fiber tube profiles and varying gear ratios. Harmonic drives are used as the gearbox between the motor input and actuator output. Our choice of a harmonic drive transmission solution is justified by their advantages including being backlash-free, lightweight, having high gear ratios for their backdrivability, high resolution, reliability, repeatability, and high torque output. A comparison between the component sets and standard transmission gear-based solutions would reveal that large gear reductions are possible in the same space in which planetary gears typically only produce a limited gear ratio. In order to eliminate the need for metal fasteners or other retaining hardware in these actuators as much as possible, components such as bearings and the harmonic drive circular spline are embedded during the composite additive manufacturing process. Two carbon fiber plates are embedded within the frontal hip actuators in order to form a strong and lightweight connection between the two without the need for fastening hardware. These plates also have an embedded 3D printed component that connect the lower body to the upper body frame with two carbon fiber rods.

Schübeler DS-30-AXI HDS impellers were chosen as the thrusters of the robot. Weighing just 55 g and producing up to 27 N of thrust, they can provide extremely large forces relative to their weight, making them optimal for our high power density robot. The pitch angle of the thrusters are each controlled by actuators which mounted to the upper body frame with carbon fiber tubes.

